Lightweight Task Offloading Exploiting MPI Wait Times for Parallel Adaptive Mesh Refinement

Balancing the workload of sophisticated simulations is inherently difficult, since we have to balance both computational workload and memory footprint over meshes that can change any time or yield unpredictable cost per mesh entity, while modern supercomputers and their interconnects start to exhibit fluctuating performance. We propose a novel lightweight balancing technique for MPI+X to accompany traditional, prediction-based load balancing. It is a reactive diffusion approach that uses online measurements of MPI idle time to migrate tasks temporarily from overloaded to underemployed ranks. Tasks are deployed to ranks which otherwise would wait, processed with high priority, and made available to the overloaded ranks again. This migration is non-persistent. Our approach hijacks idle time to do meaningful work and is totally non-blocking, asynchronous and distributed without a global data view. Tests with a seismic simulation code developed in the ExaHyPE engine uncover the method's potential. We found speed-ups of up to 2-3 for ill-balanced scenarios without logical modifications of the code base and show that the strategy is capable to react quickly to temporarily changing workload or node performance.

==> 10_artifact_description.tex <==
%TODO!


==> cover_letter.tex <==
Dear Prof. Walker,

With the present submission, we are pleased to share a manuscript on a novel
idea for load balancing. While we demonstrate the value of this idea through 
our ExaHyPE framework (www.exahype.org) - ExaHyPE allows users to solve
hyperbolic systems of partial differential equations in parallel on dynamically adaptive meshes
through a high-order explicit time stepping scheme - we think the proposed
method is of interest to a larger audience using various numerical schemes on
parallel computers and relying on high performance: Our reactive 
diffusion-based load balancing approach is orthogonal to classical geometric 
problem decomposition and acts as a second level of load balancing targeted at 
dealing with rather unpredictable performance factors at runtime, thus preparing
ExaHyPE (and readers picking up our ideas) for future systems where hardware
variability is expected to increase. Our method improves performance by
dynamically offloading tasks between MPI ranks in a very fine-grained and lightweight manner.
Given these details, we hope our manuscript is a fit to Concurrency and
Computation.


We are happy to confirm that this manuscript is not submitted anywhere else. 
We should however clarify that we had submitted an earlier version to this year's
SC Conference where it had been rejected, receiving both positive and critical reviews. 
The present text is substantially revised with the feedback from SC19 considered 
and is supplemented with additional data. 


As potential reviewer for this work, we would like to suggest Prof. Dr. Olaf 
Schenk (USI Lugano) due to his expertise in parallel software for high 
performance computing. Due to similarities in the underlying mindset around
load balancing - which we discuss in the paper - Prof. Martin Berzins from Utah
would be a fit as well. Finally, we have recently attended talks about dynamic
task graphs by Hatem Ltaief from KAUST who might be an appropriate reviewer,
too.

We look forward to sharing this work with the scientific community in high performance computing and computational sciences.

Kind regards,
Philipp Samfass, Tobias Weinzierl, Dominic E. Charrier and Michael Bader


==> data/efficiency-without-stealing.tex <==

\begin{table}
\caption{
  Shared memory parallel efficiency of our baseline code on one node without any
  offloading. 
  We start from a $25 \times 25 \times 25$ grid and then add additional levels
  of (static) AMR. We measured the baseline using $2$ threads.
  \label{table:shared_mem_efficiency}
}
\centering
\begin{tabular}{r|rr|rr}
\hline
 & \multicolumn{2}{c|}{Regular grid} & \multicolumn{2}{c}{One AMR level} \\
Threads & \added[id=CCPE1]{15626 cells} & Speedup & \added[id=CCPE1]{58525 cells} & Speedup \\
\hline 
4 & & 1.00 & & 1.00 \\
7 & & 0.97 & & 0.97 \\
14 & & 0.93 & & 0.87 \\
28 & & 0.53 & & 0.48 \\
\hline 
\end{tabular}
\end{table}

